An Analysis of Adversarial Attacks and Defenses on Autonomous Driving Models

Nowadays, autonomous driving has attracted much attention from both industry and academia. Convolutional neural network (CNN) is a key component in autonomous driving, which is also increasingly adopted in pervasive computing such as smartphones, wearable devices, and IoT networks. Prior work shows CNN-based classification models are vulnerable to adversarial attacks. However, it is uncertain to what extent regression models such as driving models are vulnerable to adversarial attacks, the effectiveness of existing defense techniques, and the defense implications for system and middleware builders. This paper presents an in-depth analysis of five adversarial attacks and four defense methods on three driving models. Experiments show that, similar to classification models, these models are still highly vulnerable to adversarial attacks. This poses a big security threat to autonomous driving and thus should be taken into account in practice. While these defense methods can effectively defend against different attacks, none of them are able to provide adequate protection against all five attacks. We derive several implications for system and middleware builders: (1) when adding a defense component against adversarial attacks, it is important to deploy multiple defense methods in tandem to achieve a good coverage of various attacks, (2) a blackbox attack is much less effective compared with a white-box attack, implying that it is important to keep model details (e.g., model architecture, hyperparameters) confidential via model obfuscation, and (3) driving models with a complex architecture are preferred if computing resources permit as they are more resilient to adversarial attacks than simple models.

==> methodology.tex <==
% \begin{figure*}[ht]
% \centering
% \includegraphics[width = .8\textwidth]{images/malware_attack.png}
% \caption{The malware cause adversarial attack on the autonomous driving model}
% \label{fig:malware-attack}
% \end{figure*}

\section{Methodology}
% \subsection{Adversarial attack threat model on autonomous driving}
% \subsection{Threat Model}
%In this section, we elaborate how remote attackers can perform adversarial attacks on autonomous driving models in real-life scenarios. 
%To avoid vehicle recall cost, autonomous vehicles are connected to the Internet and upgrade their software and firmware over the air (OTA), which allows remote attackers to intrude autonomous vehicles and inject malware~\cite{othmane2015survey}. One common scenario is to intercept the OTA upgrade packages and directly inject malware into the packages~\cite{ota}. In another scenario, since autonomous vehicles allow users to connect their mobile devices via Bluetooth or WiFi, attackers can use hacked mobile devices to transfer malware into autonomous vehicles~\cite{v2v}. %Once the malware is injected, it could be used to implement adversarial attacks. As we introduced before, the autonomous driving model is in the perception module and accepts inputs from the sensing module. 
%If the malware is injected between the sensing module (e.g., cameras) and perception module (a CNN based autonomous driving model), it is able to intercept the input images and feed adversarial images into the autonomous driving model, as shown in Figure~\ref{fig:malware-attack}.
%{\color{red}looks like we miss a figure to show the sensing module and the perception module. you can use the Tsinghua figure in our last survey}. 
%In this way, adversarial attacks could make autonomous driving models fail and output wrong predictions.
% Recently, it is reported that, by injecting malware to generate adversarial examples {\color{red}I think the malware is for remote control not for generate adversarial example, please confirm}, researchers can successfully interfere or to some extend control Telsa Model S without connecting to the vehicle physically or remotely~\cite{TelsaR}. 

%Based on the assumption of malware injection, we could discuss the adversarial attack threat model on autonomous driving models like other normal adversarial attack tasks on classification models. For adversarial attacks under white-box setting, attackers know the details of autonomous driving models including the training dataset, network architecture and parameters. Therefore, they can implement adversarial attack methods on the malware.
%With availability of the above-mentioned malware injection, 
%Similar to adversarial attacks on image classification models, adversarial attacks on autonomous driving models can be performed in both white-box and black-box settings. %In the white-box setting, attackers know all details of a driving models, including the training dataset, the network architecture, and parameters. Attackers can also run the model and gather gradients and prediction results in real time. 
%In the white-box setting, fast-gradient-based methods and optimization-based methods can be easily integrated within malware to generate adversarial images in real time, since attacker can access the calculation of gradients and prediction results of a driving model in real time.
%Therefore, fast-gradient-based methods and optimization-based methods can be easily integrated within malware to generate adversarial images in real time by utilizing the autonomous driving model running status. 
%Regarding generative-network based methods, 
%and image-independent attacks,
%attackers can first train an adversarial image generator offline using the same training dataset of a driving model %or construct the universal perturbation on the training dataset 
%and then integrate the generator into malware for real-time attack. Furthermore, given the training datatset of a driving model, attackers can also carefully design {\em universal perturbation}~\cite{moosavi2017universal} to craft adversarial images. We discuss the implementation details of these attacks in Section~\ref{sec:attack-details}. In the black-box setting, since attackers can only observe the prediction results of a driving model, they can train their own models based on the observed data offline and reuse these adversarial examples generated from their own models to attack the original model. In this study, we perform blackbox attacks by reusing adversarial examples generated from one driving model to attack another model (detailed in Section~\ref{sec:rq2}).

% Then attackers could apply some white-box adversarial attack methods to generate an universal adversarial perturbation or build a generation model to generate adversarial examples, which methods will be introduced in detail in the next section. The universal adversarial perturbation or adversarial example generator is upload to the malware. When those process are finished, the malware could intercept the images from cameras before they are feeding into the autonomous driving model in the perception module. Then it could instantly generate the adversarial example of the current image by adding universal perturbation on it or generating the adversarial example based on it using the generator. Under black-box setting, attackers could firstly train an autonomous driving model by themselves and then get the universal perturbation or adversarial example generator like the above demonstrated. Because of the transferability of adversarial examples, the universal perturbation and adversarial example generator may still work on the autonomous driving model in the vehicle. 
\subsection{Adversarial Attacks on Autonomous Driving Models}
\label{sec:attack-details}

%\todo{Tianyi: let's not spend too much space on something that is well-known in adversarial attacks. So let's keep the following descriptions simple.}
%For a standard classification model \(f\), there are two kinds of adversarial attacks: non-targeted attack and targeted attack. Non-targeted attack methods generate an adversarial example \(x + \epsilon\) that is classified as any different class from the original class \(c\), as shown in Formula (\ref{adv_clf_nt}). Targeted attack methods generate an adversarial example that are classified as the specific class \(c'\) that is different from the original class \(c\).
%\begin{equation}
%\label{adv_clf_nt}
%f(x + \epsilon) \neq c
%\end{equation}
%\begin{equation}
%f(x + \epsilon) = c'
%\end{equation}
 For an image classification model \(f\), an adversarial attack is considered successful if an adversarial image \(x + \epsilon\) is classified as a different class compared with the original image \(x\). However, autonomous driving models are regression models that predict as continuous values.
 %. Their predictions are continuous values rather than discrete class labels. 
%  When the input \(x\) changes, the prediction \(f(x)\) will always change, which satisfies the definition of non-targeted attacks on classification models but may not represent a meaningful attack on regression models. 
Therefore, adversarial attacks on driving models are defined with respect to an acceptable error range \(\Delta\), which could be called as an {\em adversarial threshold}. %For example, on a straight highway the autonomous driving model could predict current steer angle in a range as long as the vehicle could keep the straight direction. However, once the prediction is out of the range, we could think the prediction is wrong. Therefore, we could construct an image \(x + \epsilon\)  to make the deviation between normal prediction \(f(x)\) and prediction \(f(x+\epsilon)\) reach above a threshold \(\Delta\), which we call 
%\textit{adversarial threshold}. Based on this idea, an adversarial attack on regression models is defined in Formula (\ref{adv_reg}).
Hence, an adversarial attack on a driving model is considered successful if the deviation between the original prediction and the prediction of an adversarial example is above a given threshold, as shown in Formula (\ref{adv_reg}).
\begin{equation}
\label{adv_reg}
|f(x + \epsilon) - f(x)| \geq \Delta
\end{equation}
%Same as 
%Similar to adversarial attacks on classification models, there are three categories of adversarial attacks on regression models regarding the perturbation generation methods. 
In this study, we implement five adversarial attack methods{color{red}, listed below. }%lists below
These five attacks could comprehensively experiment the performances of autonomous driving models {\color{blue}as they cover three mainstream types of adversarial attacks including Fast Gradient Sign based method~\cite{goodfellow2014explaining}, Optimization based method~\cite{szegedy2013intriguing} and Generative model based method~\cite{poursaeed2018generative}, as well as an universal attack~\cite{moosavi2017universal}}.
%in these three categories 
% for regression models. For fast-gradient-based methods, we implement Iterative Targeted Fast Gradient Sign Method (IT-FGSM)~\cite{kurakin2016adversarialphysical, kurakin2016adversarial}. For optimization-based method, we implement both the original optimization based approach~\cite{szegedy2013intriguing} and the universal perturbation attack~\cite{moosavi2017universal}. For generative-network-based methods, we implement advGAN attack~\cite{xiao2018generating} and advGAN based universal perturbation attack~\cite{poursaeed2018generative}. We cannot adapt adversarial attack methods such as C\&W attack~\cite{carlini2017towards} and DeepFool~\cite{moosavi2016deepfool} to regression models. Because the calculation of adversarial perturbations in these methods relies on logits (i.e. the outputs of the second last layer of the classification model) and the softmax function, which only exist in classification models. 

% For those five adversarial attack methods, their application scenario on autonomous driving models could be classified as two type. IT-FGSM and optimization-based approach generate adversarial images based on the gradients and loss with respect of input images, which means when we apply those methods on the malware, the malware should be able to control the workflow of autonomous driving models: The malware should firstly feed the original image into autonomous driving models, get the gradient and loss information it needs, drop the original prediction, construct the adversarial image and re-feed it into autonomous driving models to implement the attack.  

%\vspace{1mm}
\subsubsection{Iterative Targeted Fast Gradient Sign Method} Iterative Targeted Fast Gradient Sign Method (IT-FGSM)~\cite{kurakin2016adversarialphysical, kurakin2016adversarial} is a variant of Fast Gradient Sign Method (FGSM), which is a classic adversarial attack method proposed by Goodfellow et. al~\cite{goodfellow2014explaining}. FGSM simply adds the sign of the loss gradient with respect to each pixel on original images. % as shown in Formula (\ref{fgsm_eq}). 
Based on FGSM, Kurakin et al.~\cite{kurakin2016adversarial} proposed targeted-FGSM.% as shown in Formula (\ref{t-fgsm}). 
%\(J_\theta\) is the Mean Squared Error (MSE) loss function to measure the loss between prediction on original images and on adversarial examples.
%\begin{equation}
%\label{t-fgsm}
%    x' = x - \epsilon \, sign(\nabla J_\theta(x, c'))  
%\end{equation}
In this study, we implement an advanced method called Iterative Targeted FGSM (IT-FGSM)~\cite{kurakin2016adversarialphysical}. IT-FGSM applies targeted FGSM multiple times to get a more powerful adversarial example, as shown in Formula~\ref{it-fgsm}. \(x'_{N+1}\) is the final adversarial example of image \(x\). 
% use \texttt font for function names and use the math mode $$  for symbolic variables and numbers
The \texttt{Clip} function 
%on intermediate results 
is to ensure that the intermediate adversarial example is always a valid image with every pixel value in the range 0 to 1. 
\begin{equation}
\label{it-fgsm}
\left\{
    \begin{array}{lr}
    x'_0\,=\,x, \\ x'_{N+1} = Clip\{x'_N - \epsilon\,sign(\nabla J_\theta(x'_N, f(x) + \Delta)\}
    \end{array}
\right.
\end{equation}

\subsubsection{Optimization Based Approach} Optimization Based Approach (OBA) is another classic method proposed by Szegedy et al. in~\cite{szegedy2013intriguing}, which is the first paper to systematically research adversarial examples. OBA calculates adversarial perturbation \(\epsilon\) for classification models by solving the optimization problem as in Formula (\ref{lbfgs})~\cite{szegedy2013intriguing}.
\begin{equation}
\label{lbfgs}
\argmin_{\epsilon}||\epsilon||_2  \hspace{3mm}s.t. \hspace{2mm}f(x+\epsilon)=c',x+\epsilon \in[0,1]^m
\end{equation}

For regression models, we only need to change \(c'\) to \(f(x) + \Delta\). In this study, we adapt Formula (\ref{lbfgs}) to create Formula (\ref{opt-based}) and apply Adam optimizer \cite{kingma2014adam} to solve the following optimization problem.
\begin{equation}
\label{opt-based}
\argmin_{\epsilon}\hspace{1mm}||\epsilon||_2+J_{\theta}(Clip(x+\epsilon),f(x) + \Delta)
\end{equation}
% Currently many targeted adversarial attack methods have been proposed but not all of them could be applied on a regression models like autonomous driving models because several targeted attack methods generate adversarial examples by solving optimization problems of maximizing the probability of classifying the adversarial example as the target class or minimizing   

\subsubsection{AdvGAN}
AdvGAN~\cite{poursaeed2018generative} is a novel attack to generate more natural adversarial examples that are imperceptible to humans by leveraging the power of generative adversarial networks (GANs). The basic idea of GAN is to train a generator network for generating images and a discriminator for judging the validity of the input images. When the discriminator cannot distinguish images between a dataset and those from a generator, the generator could generate fake images similar to real images. %The training process of GAN is implemented by minimizing the objective function shown in Formula (\ref{GAN}):
%\begin{equation}
%\label{GAN}
   % \mathcal{L}_{GAN} = \mathbb{E}_x log(\mathcal{D}(x) + \mathbb{E}_x log(1 - \mathcal{D}(\mathcal{G}(x)))
%\end{equation}  

AdvGAN generates adversarial examples \(\mathcal{G}(x)\) from original images by integrating another objective  \(\mathcal{L}_y = J_\theta(\mathcal{G}(x), f(x) + \Delta)\).%into the original objective function in Formula (\ref{GAN}). %In addition, AdvGAN introduces \(\mathcal{L}_{hinge}\) to constrain the L2 norm of perturbation.
In this study, we use the \texttt{Clip} function to directly constrain perturbation. Therefore, the objective function of training AdvGAN is shown as Formula (\ref{AdvGAN}), where \(\alpha\) sets the importance of each objective. 
\begin{equation}
\label{AdvGAN}
    \mathcal{L}_{AdvGAN} = \mathcal{L}_y + \alpha \mathcal{L}_{GAN}
\end{equation}  

Finally, Universal Adversarial perturbation and AdvGAN Universal Adversarial Perturbation are two special attacks that could generate single adversarial examples to attack the whole dataset based on Optimization Based Approach and AdvGAN. 

\subsubsection{Universal Adversarial Perturbation}
Moosavi-Dezfooli et al.~propose an approach that generates one single perturbation called universal adversarial perturbation that causes the target model to fail on most input images in the dataset~\cite{moosavi2017universal}.% The universal adversarial perturbation \(v\) should meet two constraints: \(||v||_p < \rho\) and the attack success rate achieves a certain value \(1-\delta\) on training dataset. 
In this study, we implement universal adversarial perturbation as an optimization-based approach. We first generate a perturbation \(v\) on one image. Then for each image in the dataset, we calculate the minimal change \(\Delta v\) and adapt \(v\) to \(v + \delta v\). When iterating the whole dataset, an universal perturbation is obtained. 
% The universal perturbation \(v\) is initialized as \(0^m\) where \(m\) is the total dimension of all pixels in an image. Then for each image in the training dataset, the minimal change \(\Delta v\) is calculated by solving the optimization problem as shown in Formula (\ref{universal}). 
% \begin{equation}
% \label{universal}
% \argmin_{\epsilon}\hspace{1mm}||\epsilon||_2+J_{\theta}(Clip(x+v+\Delta v),f(x) + \Delta)
% \end{equation}
% Then the universal perturbation \(v\) is updated to \(v + \Delta v\). To ensure \(v\) meets constraint \(||v||_p < \rho\), \(v\) still needs to be updated to \(v'\) by solving the following optimization problem (\ref{constraint}):
% \begin{equation}
% \label{constraint}
% argmin_{{v'}}||v'-(v+\epsilon)||_2 \hspace{5mm} s.t. ||v'||_p<\rho
% \end{equation}

\subsubsection{AdvGAN Universal Adversarial Perturbation}
Poursaeed et al.~propose to use GAN to generate universal adversarial perturbations~\cite{poursaeed2018generative}. Instead of using a generator to construct a unique perturbation \((\mathcal{G}(x))\) for each input image, they first sample a random Gaussian noise \(n \in \mathcal{N}\) with the same size as original input images. Then the generator outputs a universal adversarial perturbation \((\mathcal{G}(n))\). Therefore, adversarial examples are formed by \(\mathcal{G}(n) + x\). In this study, we also implement this approach based on AdvGAN architecture.

\subsection{Adversarial Defensessudo  usermod -aG sudo username on Autonomous Driving Models}
\label{sec:adv_defense}
%With the development of adversarial attack methods, several kinds of adversarial defense methods are also proposed to defend adversarial attacks like the section II introduced. For adversarial defense on autonomous driving models, we find that many defense methods are not available when we analyze existing 
%%categories of 
%defense methods for autonomous driving models. 
% We implement two existing defensive methods, adversarial training~\cite{goodfellow2014explaining}  and defensive distillation~\cite{papernot2016distillation}, for autonomous driving models.
While there is a proliferation of defense methods against adversarial attacks, many of them are designed for image classification tasks only and thus do not apply to regression-based autonomous driving models.
For example, adversarial transformation proposed by \cite{guo2017countering} defends adversarial attacks by randomly clipping and rotating input images. Such image transformations may not have much influence on prediction in image classification tasks. However, they will significantly influence the prediction result of regression models. 
{\color{blue} Also, adversarial de-noiser~\cite{shen2017ape} that proposes to use GAN to transform adversarial images back to normal images has the same problem of affecting predictions on original input images.} Furthermore, some adversarial detection methods~\cite{zheng2018robust, lu2017safetynet} propose to train another neural network to detect adversarial examples. Both approaches require to deploy an auxiliary model on an autonomous vehicle, which might not be practical since autonomous vehicles are resource-constrained.

{\color{blue} In this paper, 
we adapt and re-implement five adversarial defenses that are suitable for deep learning regression model and autonomous driving tasks. \textit{Adversarial training}~\cite{goodfellow2014explaining} and \textit{defensive distillation}~\cite{papernot2016distillation} are two classic defenses for adversarial attacks.  we postulate that real-time adversarial example generation might also lead to a resource usage spike in autonomous vehicles. Therefore, inspired by our prior work on runtime monitoring of autonomous systems~\cite{zheng2018efficient}, we investigate an \textit{anomaly detection} mechanism by monitoring hardware usage rates in autonomous vehicles. \textit{Feature squeezing}~\cite{xu2017feature} is an adversarial detection method that does not need an auxiliary model. 

%we adopt and re-implement five adversarial defenses that are suitable for deep learning regression model and autonomous driving tasks. \textit{Adversarial training}~\cite{goodfellow2014explaining} and \textit{defensive distillation}~\cite{papernot2016distillation} are two classic defenses for adversarial attacks.  we postulate that real-time adversarial example generation might also lead to a resource usage spike in autonomous vehicles. Therefore, we further investigate a new \textit{anomaly detection} mechanism by monitoring hardware usage rates in autonomous vehicles. \textit{feature squeezing}~\cite{xu2017feature} is an adversarial detection method that does not need auxiliary model. 
} 
 %Therefore, applying proactive methods to improve the robustness of driving models on adversarial images seems most applicable. 
\subsubsection{Adversarial Training}
%As the most common defense method, adversarial training essentially augments the original training dataset with generated adversarial examples. 
By retraining the original model with adversarial examples, the new model learns features of adversarial examples and thus has better generalization and robustness. In this study, we first use our implemented attacks to generate adversarial examples and then train a new model using the objective function shown in Formula~(\ref{adv_training}). 
%which introduces the loss of adversarial examples as an regularizer~\cite{goodfellow2014explaining}. 
This objective function enforces the training process to minimize not only prediction loss on original images but also on adversarial examples so the model could learn the features of adversarial examples and predict correctly on them.
\begin{equation}
\label{adv_training}
    \mathcal{L} = \alpha J_\theta(x, y) + (1 - \alpha) J_\theta(x', y)
\end{equation}  

\subsubsection{Defensive Distillation}
Defensive distillation is a well-known adversarial defense method for classification models~\cite{papernot2016distillation}.
% Originally, distilling is proposed by Hinton et al.~\cite{hinton2015distilling} to reduce a large, complex model to a small-scale model. Furthermore, their experiments show that the distillation method can improve model's generalization. Based on this property, Papernot et al.~further demonstrate that distillation can be used to defend against adversarial attacks~\cite{papernot2016distillation}. 
The original defensive distillation approach is designed for neural network classifiers, which use the class probabilities predicted by the original model as soft labels to train a new model. However, since autonomous driving models are regression models, they do not have class probabilities. 

%Defensive distillation is an adversarial defense method for classification models proposed in \cite{papernot2016distillation}. Distilling information from a complex model and using the information to re-train a small-scaled model was proved successful by Hinton et al.\cite{hinton2015distilling}. Furthermore, their experiments showed that the distillation method can improve model's generalization. It has been proved by Papernot et al. \cite{papernot2016distillation} that distillation can be used as adversarial defence approach for Deep Neural Networks. Previous works focused more on DNN classifiers, which use the class probabilities predicted by the original model as the soft labels to train the new model. As we are defending for a regression model, we don't have information like class probabilities, thus we need to distil other information from the original model. In the research work of Autoencoders, Hinton et al.\cite{hinton2006reducing} showed how the output of a neural network hidden layer contains information. For deep CNN regressors with fully connected (FC) layers, the outputs of FC layers contain highly encoded information that are passed from previous convolutional layers, it’s possible to perform distillation by using the output of FC layers of a deep CNN regressor as the target value. 
We adapt the original defensive distillation approach to handle regression-based driving models based on %previous findings of 
the finding by Hinton et al.~\cite{hinton2006reducing}. They show that the output of a neural network hidden layer contains highly encoded information that can be leveraged for model distillation. Similarly, the outputs of fully connected layers can be leveraged to perform defensive distillation on CNN based driving models. We observe that for inputs \(x_i\) that have similar outputs \(f(x_i)\), there are indeed uncorrelated features in the last fully connected layer outputs \(z_i^d\), which can provide additional information to distill and train a new model \(g\). While training the distilled model, we add a distillation penalizing term when computing the loss as shown in Formula~(\ref{distillation_r}), which uses the L2 distance between \(z^d\) and \({z'}^d\) as a regularizer to distill the information from the original model. \(\lambda\) is the parameter (i.e., temperature) to control the extent of distillation. In this way, we use information from both the output \(f(x)\) and the tensors \(z^d\) to train the distilled model to enhance its generalization and robustness against adversarial attacks. %Even though the implementation is different from the defensive distillation for classification models, we keep the fundamental feature of this technique that distill information from the original model to train a new model with better generalization and robustness. Therefore, we still call our implementation as defensive distillation for autonomous driving models.

\begin{equation}
\label{distillation_r}
\mathcal{L} = \Sigma_1^n(\lambda(||z_i^d - {z'_i}^d||) + ||f(x_i) - g(x_i)||)/n
\end{equation}

\subsubsection{Anomaly Detection}
%Normally on an autonomous vehicle there is an anomaly detection system to monitor the status of the vehicle whether it is under the normal condition. Therefore, we could use the below anomaly detection system to analyze whether the autonomous driving model is under adversarial attack.

Autonomous vehicles are usually equipped with a runtime monitoring system to check the vehicle state~\cite{watanabe2018runtime, zheng2018efficient}. First, a vehicle runs into an abnormal state if the driving model fails to make real-time predictions. Similarly, we monitor the model prediction time to detect any prediction delay caused by adversarial attacks. Second, since autonomous vehicles are resource-constrained, we monitor any spikes in GPU memory usage and GPU utilization rate via Nvidia System Management Interface (Nvidia-smi) to detect additional computation caused by adversarial attacks. 
%it will also cause driving prediction to slow down, this abnormal state could be detected by the anomaly detection system. 
We evaluate the effectiveness of this anomaly detection approach by comparing the prediction time per image and GPU usage with and without adversarial attacks and further investigate its effects on different kinds of attack methods. %By comparing the results we could figure out whether the anomaly detection system is able to detect adversarial attacks.
% To calculate the prediction time per image, we monitor the total time of model prediction for test set and then calculate the average prediction time for each image. We collect the GPU memory usage and GPU utilization during the model prediction on test set by Nvidia System Management Interface (Nvidia-smi) and calculate the average values 

{\color{blue}
\subsubsection{Feature squeezing}
Feature squeezing is an adversarial example detection method proposed by Xu et. al~\cite{xu2017feature}. They propose two squeezing methods which reduce the color depth and apply spatial smoothing to process input images. For color depth reducing, they squeeze the original 24-bit color down to 1-8 bit color. By doing so, adversarial noise becomes more perceptible as the bit depth decrease. For spatial smoothing, median smoothing method is proven most effective, which uses a filter across an original image and modifies the center pixel value to the median of the pixel values in the filter. For a given input image they prepare one squeezed image for each of the two methods described above, and feed the original image and the squeezed images into the same prediction model and get the results. If the difference between the prediction result of the original image and that of the squeezed image by either method exceeds a pre-defined threshold \(T\), the given input is likely to be an adversarial example.
%Feature squeezing is an adversarial example detection method proposed by Xu et. al~\cite{xu2017feature}. They propose two squeezing methods including reducing the color depth and applying spatial smoothing to process the input image. For color depth reducing, they squeeze the original 24-bit color down to 1-8 bit color and adversarial noise becomes more perceptible when the bit depth decrease. For spatial smoothing, median smoothing method is proven most effective, which slides a filter across an original image and modifies the center pixel value to the median of the pixel values in the filter. For a given input image they prepare one squeezed image for each of the two methods described above, and feed the original image and the squeezed images into the same prediction model and get the results. If the difference between the prediction result of the original image and the prediction result of either squeezed image exceeds a pre-defined threshold \(T\), the given input is likely to be an adversarial example.
}

% \subsubsection{Numerical Stability Regularization}
% Numerical Stability Regularization was proposed in~\cite{nguyen2018adversarial}. this method regularizes the deep learning model to improve the numerical stability that the predictions should be similar if two inputs are near each other. In the training phase, the method samples several neighbors for each input by randomly adding small perturbations on the input and expects the predictions of neighbors should as close as possible to the prediction of the input. The mean difference between the predictions of input and neighbors is the numerical stability loss as the regularization to improve the robustness of deep learning models for adversarial attacks. }

==> related_work.tex <==
\section{Related Works}

\textbf{Adversarial Defenses}
%Adversarial attacks on deep learning classifier models are firstly introduced by Szegedy et al.\cite{szegedy2013intriguing}. They use optimization-based attack method to generate adversarial examples. Goodfellow et al. {\color{red}citation needed} invented FGSM method to reduce attack computation time as compared to optimization based methods. FGSM based approaches normally require a small number of iterations to generate adversarial examples. The FGSM method has been extended to Targeted-FGSM and Rand-FGSM {\color{red}citation needed, you also need to include one sentence to introduce what are the key features of these extension}. The optimization based attacking method proposed by Szegedy et al. has also been extended into a few new attacks. For example, Su et al. \cite{su2019one} proposed the One pixel attack method, which only changes one pixel in each input image to fool a DNN classfier model. %Different from methods introduced above in this paragraph, 
%Moosavi-Dezfooli et al. \cite{moosavi2017universal} proposed the Universal Perturbation attack, which generates only one perturbation image for all input images. 
%Generative models are also used for adversarial attacks. In \cite{baluja2017adversarial} Baluja et al. utilized Autoencoder archetecture to generate perturbations to perform attacks. After Generative Adversarial Network (GAN) was proposed, Xiao et al. used GAN to generate perturbation {\color{red}citation needed}. Benefited by the nature of GAN, the generated examples are very similar to the input images and thus are difficult to be detected. 
Several techniques have been proposed to defend adversarial attacks, which can be roughly categorized as proactive defense and reactive defense. 
Proactive defense aims to improve the robustness of a neural network against adversarial examples.
%~\cite{goodfellow2014explaining, papernot2016distillation, yan2018deep}. 
Goodfellow et al.~propose {\em adversarial training} that retrains the driving model by augmenting its training set with adversarial examples~\cite{goodfellow2014explaining}. 
Papernot et al.~introduce {\em defensive distillation} that increases the magnitude of the inputs to the softmax layer by adjusting a parameter $T$ called "Temperature" into the standard softmax function to harden a neural network~\cite{papernot2016distillation}.
In~\cite{yan2018deep}, network regularization is introduced to achieve better generalization of a target model by adding another penalization term to the original loss function, or by adding regularization components to the target model.

Reactive methods, on the other hand, aim to detect adversarial examples, rather than improving the robustness of a neural network. 
%The main reactive defense techniques are adversarial detection, adversarial transformation and adversarial denoising. 
Zheng et al.~\cite{zheng2018robust} propose to train another neural network as a detector to verify the properties of input images and detect adversarial examples. 
%Adversarial transformation methods such as~\cite{guo2017countering} aim to apply multiple image transformations such as image re-scaling, image cropping, and image compression to remove adversarial features in an adversarial example.
Adversarial denoising leverages GAN to transform adversarial images back to original images~\cite{shen2017ape}.
%Some works adopted anomaly detection methods for adversarial defence: 
Lee et al.~propose an effective way to detect abnormal samples on a DNN classifier model with a softmax layer by using Gaussian discriminant analysis~\cite{lee2018simple}. 
%Some other works tries to pre-process input images using different approaches: 
%Dziugaite et.al \cite{dziugaite2016study} proved that using JPG compressing technology to process the adversarial samples can lower the attacking success rate if the perturbations are rather small.
%Liao et al.\cite{liao2018defense} proposed a High-Level Representation Guided Denoiser. They used Autoencoder architecture, but they changed the loss function of the Autoencoder from \(L2\) norm of the network output difference to network layer-wise output difference. 
Compared to our work, these techniques all focus on analyzing attacks on classification models. Our work investigates attacks and defenses on regression models, extending and experimenting with existing attack and defense techniques to autonomous driving.
%as shown below. %At first a deep learning model is trained based on original inputs \(X\) and labels \(y\). The output of the model is probability logits of inputs \(f(X)\) calculated by a softmax function with temperature \(T\).
%\begin{equation}
%\label{distillation}
%f(X) = \frac{exp (z_i(X)/T)}{\sum_j exp 5(z_j(X)/T)}
%\end{equation}
%Here $z$ are the activations of the last layer before the softmax layer. $T=1$ is equivalent to standard softmax, while increasing $T$ has the effect of pushing the resulting probability distribution closer to uniform. The intuition is to train a more flexible neural network that can still make correct predictions on perturbed input.
%Then \(X\) and \(f(X)\) are used to train another same architecture model with the same temperature \(T\). The new distilled model is the final model used for prediction. This method could work because the new model has better generalization among data points than previous model \cite{papernot2016distillation}.


%{\color{red}check below works and confirm whether they are proactive defense}
%Gu et al. \cite{gu2014towards} used the Deep Contractive Network model, which have a special designed loss function penalization term. Instead of  the widely used \(L2\) norm of the weights, they use the \(L2\) norm of neural network layer-wise Jacobian Matrices. Sharing the idea of network regularization, Cisse et al. introduced the Parseval network \cite{cisse2017parseval} to control the Lipschitz constant of a NN model.


%For adversarial defenses, some measures other than those introduced in the background sections are also proven effective.
\textbf{Testing and Verification of Deep Learning Models}
%Normally we measure the quality of dlearningsystems only depending on the prediction accuracy on the provided test dataset. However,  this measurement is not enough to tell us the robustness and generality on some corner cases or adversarial examples that do not exist in the test dataset \cite{goodfellow2017challenge}. 
Recently, the software engineering community makes significant advances in testing and debugging deep learning models~\cite{pei2017deepxplore, ma2018deepgauge, 2019arXiv180808444K, sun2018concolic, tian2018deeptest, zhang2018deeproad, ma2018combinatorial}.  DeepXplore~\cite{pei2017deepxplore} introduces an effectiveness metric called neuron coverage to measure how much of the internal logic of a DNN has been tested. Based on this metric, a white-box differential testing algorithm is proposed to find inputs that cause inconsistencies between multiple DNNs. DeepTest~\cite{tian2018deeptest} and DeepRoad~\cite{zhang2018deeproad} are two techniques to generate corner-case inputs to test autonomous driving models. DeepTest applies a set of image transformations like scaling, shearing, and rotation to generate new test images to detect inconsistencies among driving models. DeepRoad relies on the power of GAN to transform road scene images to different weather conditions for testing the robustness of driving models. DeepGauge~\cite{ma2018deepgauge} presents multi-granularity testing coverage metrics for DL systems to help exploring the running status of a DNN to find defects on both major function regions and corner-case regions. Given the large test space of DNN, DeepCT~\cite{ma2018combinatorial} implements combinatorial testing derived from traditional software testing to generate a reasonable number of tests for DNN. 
%with the balance of defect detection ability.
DeepMutation~\cite{ma2018deepmutation} implements the mutation test for deep learning systems to measure the quality of the test dataset. DeepConcolic~\cite{sun2018concolic} implements concolic testing for deep learning neural networks to find adversarial examples of the networks. Wicker et al.~ \cite{wicker2018feature} propose a black-box approach to test the robustness of deep learning neural networks on adversarial examples.

Deep learning verification is also gaining momentum. 
%is applying formal verification to provide guarantees on the security of deep learning neural networks. 
Pulina et al.~propose an abstraction-refinement approach to verify the safety of a small neural network with $6$ neurons~\cite{pulina2010abstraction}. Reluplex~\cite{katz2017reluplex} is an SMT-based approach to verify the robustness of neural networks that use ReLU activation functions. Based on Reluplex, DeepSafe~\cite{gopinath2017deepsafe} identifies safe regions in the input space where a neural network is robust against adversarial perturbations. Huang et al.~propose a framework that leverages SMT and exhaustive search to find adversarial examples of a neural network~\cite{huang2017safety}.
Compared to these testing and verification techniques, our main focus is to draw a deeper understanding of attacks and defenses on autonomous driving models. We investigate the hypothesis that real-time adversarial attacks on autonomous vehicles will cause computation overhead, which can be leveraged for proactive adversarial detection. Our work identifies real risks of autonomous driving models and also discusses future directions for securing these driving models.  

%then focus on exploring the performances of adversarial examples generated by different adversarial attack methods as well as the performances of adversarial defense methods on targeted autonomous driving models.

